Stochastic Modelling of Symmetric Positive Definite Material Tensors

Spatial symmetries and invariances play an important role in the behaviour of materials and should be respected in the description and modelling of material properties. The focus here is the class of physically symmetric and positive definite tensors, as they appear often in the description of materials, and one wants to be able to prescribe certain classes of spatial symmetries and invariances for each member of the whole ensemble, while at the same time demanding that the mean or expected value of the ensemble be subject to a possibly 'higher' spatial invariance class. We formulate a modelling framework which not only respects these two requirements$-$positive definiteness and invariance$-$but also allows a fine control over orientation on one hand, and strength/size on the other. As the set of positive definite tensors is not a linear space, but rather an open convex cone in the linear space of physically symmetric tensors, we consider it advantageous to widen the notion of mean to the so-called Fr\'echet mean on a metric space, which is based on distance measures or metrics between positive definite tensors other than the usual Euclidean one. It is shown how the random ensemble can be modelled and generated, independently in its scaling and orientational or directional aspects, with a Lie algebra representation via a memoryless transformation. The parameters which describe the elements in this Lie algebra are then to be considered as random fields on the domain of interest. As an example, a 2D and a 3D model of steady-state heat conduction in a human proximal femur, a bone with high material anisotropy, is modelled with a random thermal conductivity tensor, and the numerical results show the distinct impact of incorporating into the constitutive model different material uncertainties$-$scaling, orientation, and prescribed material symmetry$-$on the desired quantities of interest.

==> application.tex <==
% !TEX root = ../paper_tensors.tex
% !TEX encoding = UTF-8 Unicode

\section{Application: heat conduction in a proximal femur}\label{Sec:Application}
%
%Let us consider a two dimensional geometry $\spatialdomain \subset \Euclideanspace$ with smooth Lipschitz boundary $\Gamma$. The following governing equations
%\begin{align}\label{Eq:DetlForm}
%-\textrm{div}(\conducttensor \cdot \nabla\temperature(x))   &= \heatsource(x),  \quad \forall x \in \spatialdomain, \nonumber \\
%\temperature(x) &= {\temperature}_0,  \quad \forall x \in \Gamma_D, \\
%(\conducttensor \cdot \nabla\temperature(x))\cdot\vek{n}(x) &= {g}(x), \quad \forall x \in \Gamma_N, \nonumber
%\end{align}
%describe the physical phenomenon of steady state heat transfer. The aim is to determine the temperature $\temperature(x) \in \mathbb{R}$ at a spatial point $x\in \spatialdomain$.
%In \feq{Eq:DetlForm}, $\Delta$ defines the Laplacian operator; $\conducttensor\in\PosSymSecRankSpacetwoD$ represents the thermal conductivity tensor; $\heatsource(x) \in \mathbb{R}$ is the heat source;  ${g}(x) \in \mathbb{R}$ represents the surface heat flux on Neumann boundary $\Gamma_N \subset \Gamma$, and $\vek{n}(x) \in \mathbb{R}^2$ is the outward unit normal to $\Gamma_N$. For simplification, a homogeneous temperature ${\temperature}_0 \in \mathbb{R}$ is considered on the Dirichlet boundary $\Gamma_D \subseteq \Gamma $. We may also further assume that $\Gamma_D \cap \Gamma_N = 0$. 
The application we have in mind is the steady-state heat conduction in bones, a highly anisotropic
material.  More specifically, we shall look at both a 2D and 3D model of the proximal femur,
this is the upper part of the thigh bone close to the hip.  Here we shall investigate the
effects of different models of the anisotropy of the heat conduction tensor
on the heat conduction and temperature distribution in the proximal femur.

Referring to the deterministic model of heat conduction defined in \feq{Eq:deterministic-thm}, 
let the conductivity tensor $\conducttensor\in\PosSymSecRankSpace$ be modelled as
a random tensor as described
%on probability space $(\samplespace,\sigmaalgebra,\probability)$
%as an exponential mapping of the model explained 
in \feq{Eq:rand-ax-rep}. 
The scaling terms $\vek{\Lambda_s}=\diag(\lambda_s^{(i)})\in\PosSymSecRankSpace$ of the 
tensor $\conducttensor$ are modelled as positive log-normal random variables:
\begin{equation}\label{Eq:lognormal}
 \vek{\Lambda_s}(\event_s) = \diag(\lambda_s^{(i)}(\event_s)) = \exp(\symdiag_s(\event_s))=
 \diag(\exp(y_s^{(i)}(\event_s))), 
\end{equation}
i.e.\ a non-linear transformation of the Gaussian random variables
\begin{equation}
    y_s^{(i)}(\event_s) \sim \normaldist(\mu_i,\sigma_i),  
      \quad i= 1, \dots, d,
\end{equation}
% \begin{equation}\label{Eq:lognormal}
% \textrm{diag}(\lambda_s(\event_s)^{(i)}) = \text{exp}({\mu_i} + \sigma_i\theta_i(\event_s)),  \quad i=\left\lbrace 1,..,d\right\rbrace,
% \end{equation}
% i.e., a non-linear transformation of standard Gaussian random variables $[\theta_i(\event_s)]^d_{i=1}$. 
where the parameters $\{\mu_i\}^d_{i=1}\in\mathbb{R}$ and $\{\sigma_i\}^d_{i=1}\in\PosRealStrict$ 
denote the mean and standard deviation corresponding to the Gaussian distribution.
% \begin{equation}
% 	 \normaldist(\mu_i,\sigma_i) \sim \log\eigvalsclele(\event_s), \quad i=\left\lbrace 1,..,d\right\rbrace.
% \end{equation}

Further, the directional uncertainty of $\conducttensor$ is accounted by modelling the 
eigenvectors in $\meaneigvect_r$ as von Mises-Fisher distributions defined on the unit sphere 
$\unitsphere$ \cite{mardia_directional_2000}. If $\rotvect$ is one of the eigenvectors of the matrix $\meaneigvect_r$, then a von Mises-Fisher unit vector $\rotvect(\event_r)$ with mean direction $\mucirc\in\unitsphere$ 
has a \acrfull{pdf} of the form:
%A von-Mises random variable $\rotangle(\event_r)$ with mean direction $\circmeananly=0$ has the \acrfull{pdf} of the form:
\begin{equation}\label{Eq:VMFPDF}
	f(\rotvect(\event_r)|\mucirc,\concparam) = 
	\frac{\concparam^{d/2-1}}{(2\pi)^{d/2}\mathcal{I}_{d/2-1}(\concparam)} 
	    \exp(\concparam \mucirc^T\rotvect(\event_r)), 
\end{equation}
where 
%$\circmeananly\in[0,2\pi)$ (note that, in this study, $\circmeananly=0$) and 
$\concparam\in\PosRealStrict$ is the measure of concentration, and $\mathcal{I}_p$ is the 
modified Bessel function of order $p$.
When $d=2$, as only the
rotational angle $\rotangle(\event_r)$ is modelled as a random variable on the unit circle $\unitcircle$, the above PDF reduces to the 
von Mises distribution \cite{best_efficient_1979}:
\begin{equation}\label{Eq:VMPDF}
f(\rotangle(\event_r)|\circmeananly,\concparam) = 
 \frac{\exp(\concparam\cos(\rotangle(\event_r)-\circmeananly))}{2\pi \mathcal{I}_0(\concparam)},
\end{equation}
in which $\circmeananly$ is the mean direction of the von Mises circular random variable 
$\rotangle(\event_r)$.
    
By rewriting the deterministic model in \feq{Eq:deterministic-thm} to a stochastic one 
\begin{equation}\label{Eq:stochastic-thm}
-\nabla\cdot(\conducttensor(\event) \nabla T(\vek{x},\event)) = 
      f(\vek{x})\quad \forall \vek{x}\in\spatialdomain, \event\in\samplespace,
\end{equation}
which has to be understood in a weak sense, both as regards the spatial as well as the
stochastic dependence.
%\begin{align}\label{Eq:StoForm}
%-\textrm{div}(\conducttensor(\event) \cdot \nabla\temperature(x,\event))   &= \heatsource(x),  \quad \forall x \in \spatialdomain, \event\in\samplespace, \nonumber \\
%{\temperature}(x,\event) &= {\temperature}_0,  \quad \forall x \in \Gamma_D, \event\in\samplespace, \\
%(\conducttensor(\event) \cdot \nabla\temperature(x,\event))\cdot\vek{n}(x) &= {g}(x), \quad \forall x \in \Gamma_N, \event\in\samplespace, \nonumber
%\end{align}
The goal is to determine the random temperature field 
$\temperature(\vek{x},\event):\spatialdomain\times\samplespace\rightarrow\mathbb{R}$, assuming deterministic boundary conditions and heat source. 

% Note that here the boundary conditions and heat source stay deterministic. 
Given the weak form of \feq{Eq:stochastic-thm}, we use the finite element method to seek 
for an approximate solution $\temperatureApprox(\vek{x},\event)$ 
on a finite-dimensional subspace $\finitespace\subset\solspace$ of the solution space $\solspace$ of \feq{Eq:deterministic-thm}, where as usual $h$ is the discretisation parameter---
an indicator of element size.
Subsequently, the objective of this study is to determine the statistics like the mean 
and standard deviation of the solution $\temperatureApprox(\vek{x},\event)$ using the 
classical Monte Carlo method (\acrshort{mc}) \cite{metropolis_monte_1949, fishman_monte_1996}.
Given, i.i.d.\ $\{\conducttensor(\event_i)\}_{i=1}^{N}$ samples, where $\samplesize$ is the 
sample size, one may compute the statistics of discretised solution 
$\stotemp:=\{\temperatureApprox(\vek{x},\event_i)\}_{i=1}^{N}$.  The unbiased sample mean
 \cite{dekking_modern_2005} is then calculated as
\begin{equation}
	\meanMC(\stotemp) := \frac{1}{\samplesize}\sum_{i=1}^{\samplesize}
	     \temperatureApprox(\vek{x},\event_i), 
\end{equation}
and the corrected sample standard deviation as
\begin{equation}
\stdMC(\stotemp) := \sqrt{\frac{1}{\samplesize-1}\sum_{i=1}^{\samplesize}
    (\temperatureApprox(\vek{x},\event_i)-\meanMC(\stotemp))^2}.
\end{equation}

Along with the temperature field, we also evaluate the heat flux vector field 
$\heatflux(\vek{x},\event):\spatialdomain\times\samplespace \rightarrow \Euclideanspace$, whose approximate solution
% By determining an approximation to the random heat flux vector field 
$\heatflux_h(\vek{x},\event)$ is determined on a finite-dimensional subspace $\solspaceheat_h\subset\solspaceheat$, where $\solspaceheat$ is the solution space of heat flux, $\heatflux(\vek{x})=\conducttensor \nabla T(\vek{x})$.
% $\heatflux_h(\vek{x},\event):\spatialdomain\times\samplespace \rightarrow \Euclideanspace$, 
Further, we determine 
the second order statistics of the magnitude of approximate heat flux vector field in the Euclidean norm i.e.\ $q_h^{(t)}(\vek{x},\event) = 
\|\heatflux_h(\vek{x},\event)\|$.
More specifically, the statistics such as the mean and standard deviation are obtained 
by sampling based MC estimators $\meanMC(\stototalflux)$ and 
$\stdMC(\stototalflux)$, respectively.
% Therefore, 
% \acrshort{mc} is implemented to evaluate the statistics of heat flux $\stoflux:=[\heatflux_h(x,\event_i)]_{i=1}^{N}$. More specifically, the mean and variance of total heat flux $\stototalflux = \|\stoflux\|$, are determined by estimators $\meanMC(\stototalflux)$ and $\varMC(\stototalflux)$ respectively.

Apart from evaluating the statistics of magnitude of heat flux field $\heatflux_h(\vek{x},\event)$, 
one may also be interested in 
understanding the statistics of direction of heat flow.
% determining the  statistics of directional aspect of the vector field. 
To this, one may compute the second order circular statistics of the normalized heat flux, 
$\hat{\heatflux}_h(\vek{x},\event) = {\heatflux_h(\vek{x},\event)}/{q_h^{(t)}(\vek{x},\event)}$.
% In addition, to estimate the circular statistics of the sampled response 
% $\stoflux:=\{\heatflux_h(\vek{x},\event_i)\}_{i=1}^{N}$ 
% \cite{mardia_directional_2000,jammalamadaka_topics_2001}, one is interested in 
% determining the orientation and not only the magnitude of $\stoflux$. 
% Thus, for convenience, the quantity $\heatflux_h$ is normalised as 
% \begin{equation}\label{Eq:normheatflux}
% 	\hat{\heatflux}_h = \frac{\heatflux_h}{q_h^{(t)}}.
% \end{equation}
%Thereby, the unit heat flux vector field $\stofluxunit$ belongs to the unit sphere 
%$ \unitsphere$.
Subsequently, the \acrshort{mc} mean estimate of sampled unit vector field 
$\stofluxunit:=\{\hat{\heatflux}_h(\vek{x},\event_i)\}_{i=1}^{N}$ 
% $\hat{\heatflux}_h(\vek{x},\event)$ 
can be estimated accordingly \cite{mardia_directional_2000,jammalamadaka_topics_2001}:
\begin{equation}\label{Eq:meannormheatflux}
	\meanMCbold(\stofluxunit) = \frac{1}{\samplesize}\sum_{i=1}^{\samplesize}
	   \hat{\heatflux}_h(\vek{x},\event_i) = L\,  \muMCcirc(\stofluxunit),
\end{equation}
where $L = \|\meanMCbold(\stofluxunit)\| \leq 1$ represents resultant Euclidean length 
of the sample mean $\meanMCbold(\stofluxunit)\in\Euclideanspace$, and 
$\muMCcirc(\stofluxunit) = \meanMCbold(\stofluxunit)/\|\meanMCbold(\stofluxunit)\|$ 
is a unit vector defining the sample mean direction of $\stofluxunit$. 
With the help of the former one, the sample circular standard deviation of $\stofluxunit$ 
can further be evaluated as
\begin{equation}\label{Eq:circvarnormheatflux}
	\stdMCcirc(\stofluxunit) = \sqrt{-2\log L}.
\end{equation}

% where $\stdMCcirc(\stofluxunit)\in[0,\infty]$.


==> results_input_2D.tex <==
% !TEX root = ../paper_tensors.tex
% !TEX encoding = UTF-8 Unicode

\begin{wrapfigure}{r}{0.39\textwidth}
	\centering
	\includegraphics[width=0.75\linewidth]{images/bc/2D_femur_BC_thermal_sideflux_1.eps}
	\captionof{figure}{Boundary conditions of 2D femur bone}
	\label{Fig:BC}	
\end{wrapfigure}
	
A two-dimensional proximal femur with a body of approximately 7 cm in width and 
21.7 cm in height is considered, see \ffig{Fig:BC}.  A uniformly distributed surface 
heat flux with a resultant heating of 0.1 W and a fixed temperature of $0\ ^\circ C$ 
are applied at locations as shown in \ffig{Fig:BC} \cite{davidson_heat_1988}. 
The computational domain is discretized by the finite element discretization 
method with 171 four-noded plane-stress elements, %see   
%\ftbl{Tbl:meshspec} for the mesh specifications. 
giving a mesh with 206 nodes and 390 degrees of freedom.
In this study, each deterministic 
simulation obtained by sampling the stochastic parametric space is solved by the 
Calculix solver \cite{Dhondt_CCX_2004}. 
For the \acrshort{mc} simulation, the %Karl 
Pearson coefficient of dispersion $\delta=0.1$ 
(for the scaling uncertainty) and  $\samplesize=10^5$ samples are considered for all the cases 
in this study.
%\begin{table}[ht]
%\centering
%	\begin{tabular}{lll}
%		\specialrule{1pt}{1pt}{1pt}			
%		Elements & Nodes & \begin{tabular}[c]{@{}l@{}}
%			Degrees of \\ freedom 
%		\end{tabular} \\ \midrule
%		171 & 206 & 390 \\  
%		\specialrule{1pt}{1pt}{1pt}
%	\end{tabular}
%	\caption{Mesh specifications of 2D femur}
%	\label{Tbl:meshspec}
%\end{table}
% \vspace{0.6cm}
% \begin{wraptable}[7]{r}{0.39\textwidth}
% 	\begin{tabular}{lll}
% 		\specialrule{1pt}{1pt}{1pt}			
% 		Elements & Nodes & \begin{tabular}[c]{@{}l@{}}
% 			Degrees of \\ freedom 
% 		\end{tabular} \\ \midrule
% 		171 & 206 & 390 \\  
% 		\specialrule{1pt}{1pt}{1pt}
% 	\end{tabular}
% 	\caption{Mesh specifications of 2D femur}
% 	\label{Tbl:meshspec}
% \end{wraptable}

For simplification, we use abbreviations defined in \ftbl{Tbl:abbreviation} which are 
used to refer different modelling scenarios considered in this study.  Each model will 
have a unique name in the form: reference tensor symmetry-realisation symmetry-type of model. 
For instance, ``iso-ortho-scl'' represents a model with random scaling only, such that the 
reference tensor belongs to isotropic symmetry, whereas the realisations are of orthotropic 
symmetry.  Three such possible scenarios are explored in this article---``iso-iso-scl'' 
(isotropy-isotropy-random scaling), ``iso-ortho-scl'' (isotropy-orthotropy-random scaling), 
and ``ortho-ortho-dir'' (orthotropy-orthotropy-random direction).
\begin{table}[h!]
	\centering 
	\begin{tabular}{llll}
	\specialrule{1pt}{1pt}{1pt}
	\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}Mean/realisation  symmetry\end{tabular}} & \multicolumn{2}{l}{Type of model}                                                                                    \\ \midrule
	isotropy                                   & orthotropy                                  & \begin{tabular}[c]{@{}l@{}}random scaling\end{tabular} & \begin{tabular}[c]{@{}l@{}}random direction\end{tabular} \\ \midrule
	\acrshort{iso}                                       & \acrshort{ortho}                                       & \acrshort{scl}                                                      & \acrshort{dir}   \\ \specialrule{1pt}{1pt}{1pt}                                                   
	\end{tabular}
\caption{Model abbreviations\label{Tbl:abbreviation}} 	
\end{table} 
Consequently, using the subscripts defined in \fsec{Ssec:group-inv-detl} for random scaling 
and random orientation, two reference conductivity tensors---
$\meanconducttensorscl\in\PosSymSecRankSpacetwoD$ belonging to the isotropic symmetry class
(denoted by superscript $iso$) and $\meanconducttensorortho\in\PosSymSecRankSpacetwoD$ 
with orthotropic symmetry (with superscript $ortho$)---are considered, whose values are 
tabulated in \ftbl{Tbl:meantensor} \cite{davidson_measurement_2000}.  
% Note that the eigenvalues of the model $\meanconducttensorortho$ are 
%$\meaneigvalscleleone=0.54$ W/mK and $\meaneigvalscleletwo=1$ W/mK.
Furthermore, we simulate the grain orientations of the femur in a spatially homogeneous 
sense. As a result, the eigenvectors of the tensor $\meanconducttensorortho$ corresponding 
to the eigenvalues $\meaneigvalroteleone$ and $\meaneigvalroteletwo$ are oriented at an 
angle of $\pi/4$ in a clockwise direction to the x and y-axis, respectively. 
\begin{table}[h!]
	\centering
	\begin{tabular}{ll}
	\specialrule{1pt}{1pt}{1pt}
	 \begin{tabular}[c]{@{}l@{}}isotropy\\ (W/mK)\end{tabular} & \begin{tabular}[c]{@{}l@{}}orthotropy\\ (W/mK)\end{tabular} \\ 
	 $\meanconducttensorscl$ & $\meanconducttensorortho$\\ \midrule 
	 $
	\begin{bmatrix}
	0.54 & 0  \\ 0 & 0.54
	\end{bmatrix} $  &  $  \begin{bmatrix}
	0.77 & 0.23  \\ 0.23 & 0.77
	\end{bmatrix} $ \\ \midrule
	\multicolumn{2}{c}{Eigenvalues (W/mK)} \\  \midrule
	\begin{tabular}[c]{@{}l@{}}$\meaneigvalscleleone=0.54$,\\ $\meaneigvalscleletwo=0.54$\end{tabular} & \begin{tabular}[c]{@{}l@{}}$\meaneigvalroteleone=0.54$,\\ $\meaneigvalroteletwo=1$\end{tabular} \\
	\specialrule{1pt}{1pt}{1pt}            
	\end{tabular}
\caption{Reference conductivity tensors with corresponding eigenvalues of 2D femur\label{Tbl:meantensor}}
\end{table}
% For simplification, we use abbreviations defined in \ftbl{Tbl:abbreviation} which refer to different modelling scenarios. Each model will have a unique name in the form: reference tensor symmetry-realisation symmetry-type of model.


\paragraph{Random scaling with fixed symmetry:}
the first modelling scenario is the one in which 
we perform random scaling only, such that 
the reference tensor $\meanconducttensorscl$, as well as the realisations, belong to 
isotropic symmetry (denoted by \acrshort{iso}-\acrshort{iso}-\acrshort{scl}); 
see \ffig{Fig:isoisoscl} for a schematic overview of the model.
In such a case, %we model 
the random tensor $\conducttensorscl(\event_s)\in\PosSymSecRankSpacetwoD$ 
%the exponential of the model depicted in \feq{Eq:rndscl}   
is modelled---as in \feq{Eq:SpecDec-rep-spl}
---with random scaling only.  Here the uncertain scaling parameters 
$\eigvalscleleone(\event_s)=\eigvalscleletwo(\event_s)$ are modelled as identical 
%and independent 
log-normal random variables. 
% \ffig{Fig:isoisoscl} presents an overview of the stochastic model $\conducttensorscl(\event_s)$, such that fixed isotropic symmetry in the mean and realisations are maintained---denoted as \acrshort{iso}-\acrshort{iso}-\acrshort{scl}. 
Their corresponding \acrshort{pdf}s are shown in \ffig{Fig:isoisoLN}. 
A geometrically equivalent (circular) representation of reference tensor and realisations 
$\{\conducttensorscl(\event_{s_i})\}^\samplesize_{i=1}\equiv\{\conducttensor_{s_i}\}^\samplesize_{i=1}$,
where the radius of circle is defined by ${1}/{\sqrt{\eigvalscleleone(\event_s)}}$ and 
${1}/{\sqrt{\eigvalscleletwo(\event_s)}}$ \cite{malgrange_symmetry_2014}, is presented 
in \ffig{Fig:isoisoquad}. 
% Note that, in this article, all the geometries representing the random tensors are 
% enhanced by scaling the eigenvalues by a factor of 0.5.
As can be seen the preservation of isotropic symmetry is apparent given the constant 
circular shape among the random variable realisations. However, 
the varying size of circles signifies 
a variation in scaling parameters.

\begin{figure}[h!]
	\centering
	\begin{subfigure}{\textwidth}
		\centering
		\input{images/input/2D_LN_iso_iso}
		\caption{}
		\label{Fig:isoisoLN}
	\end{subfigure}	
	\begin{subfigure}{\textwidth}
		\centering
		\includegraphics[width=0.7\linewidth]{images/input/2D_iso_iso_scl_v2.eps}
		\caption{}
		\label{Fig:isoisoquad}
	\end{subfigure}	
	\caption{Stochastic tensor $\conducttensorscl(\event_s)$ with fixed symmetry 
	(\acrshort{iso}-\acrshort{iso}-\acrshort{scl}): \subref{Fig:isoisoLN} log-normal 
	\acrshort{pdf} of identical random scaling values $\eigvalscleleone(\event_s) 
	=\eigvalscleletwo(\event_s)$, \subref{Fig:isoisoquad} geometric visualization of reference 
	tensor $\meanconducttensorscl$ and realisations of random tensor $\conducttensorscl(\event_s)$; 
	the geometries are enhanced by scaling the eigenvalues by a factor of 0.5} 
	\label{Fig:isoisoscl}
\end{figure}


\paragraph{Random scaling with varying symmetry:}
in the next scenario, we consider a similar stochastic tensor 
$\conducttensorscl(\event_s)\in\PosSymSecRankSpacetwoD$ as described previously with a 
similar reference tensor $\meanconducttensorscl$.  The difference being that the eigenvalues 
$\{\eigvalsclele\}^2_{i=1}$ are modelled as independent identically distributed (i.i.d.) 
log-normal random variables.  Due to which the realisations of model 
$\conducttensorscl(\event_s)$ belong to orthotropic symmetry, thus, 
this model is denoted as \acrshort{iso}-\acrshort{ortho}-\acrshort{scl}. 
Furthermore, in orthotropic realisations, the eigenvectors of $\conducttensorscl(\event_s)$ 
related to random eigenvalues $\eigvalscleleone(\event_s)$ and $\eigvalscleletwo(\event_s)$ 
are constrained at an angle of $\pi/4$ in clockwise direction with respect to x and y-axis 
respectively. 
The schematic representation of this model with varying symmetry is displayed in 
\ffig{Fig:isoorthoscl}, in which
the corresponding \acrshort{pdf}s are shown in \ffig{Fig:isoorthoLN}. 
% \ffig{Fig:isoorthoquad} presents the graphical interpretation of the model.
Closer inspection of the \ffig{Fig:isoorthoquad} shows the shift from circular geometry 
of isotropic reference tensor to orthotropic elliptical shape in realisations.  
One may also notice the variation in size of ellipses in the realisations as the 
semi-axes of ellipse are determined by ${1}/{\sqrt{\eigvalscleleone(\event_s)}}$ and 
${1}/{\sqrt{\eigvalscleletwo(\event_s)}}$.  
\begin{figure}[h!]
	\centering
	\begin{subfigure}{\textwidth}
		\centering
		\input{images/input/2D_LN_iso_ortho}
		\caption{}
		\label{Fig:isoorthoLN}
	\end{subfigure}
	\begin{subfigure}{\textwidth}
		\centering
		\includegraphics[width=0.7\linewidth]{images/input/2D_iso_ortho_scl_v2.eps}
		\caption{}
		\label{Fig:isoorthoquad}
	\end{subfigure}	
	\caption{Stochastic tensor $\conducttensorscl(\event_s)$ with varying symmetry 
	(\acrshort{iso}-\acrshort{ortho}-\acrshort{scl}): \subref{Fig:isoorthoLN} log-normal 
	\acrshort{pdf} of i.i.d.\ random scaling values $\{\eigvalsclele\}^2_{i=1}$, 
	\subref{Fig:isoorthoquad} geometric visualization of reference tensor 
	$\meanconducttensorscl$ and realisations of random tensor $\conducttensorscl(\event_s)$; 
	the geometries are enhanced by scaling the eigenvalues by a factor of 0.5}
	\label{Fig:isoorthoscl}
\end{figure}

\paragraph{Random direction with fixed symmetry:}
in the last modelling scenario, we build a random tensor $\conducttensorrot(\event_r)\in\PosSymSecRankSpacetwoD$, i.e. 
the exponential mapping of stochastic tensor as shown in
% $\conducttensorrot(\event_r)=\exp(\symtensor_r(\event_r))$ from
\feq{Eq:stomodrot}, with random orientation only, given the reference tensor $\meanconducttensorortho$. Here the model is designated as \acrshort{ortho}-\acrshort{ortho}-\acrshort{dir}, since, a fixed orthotropic symmetry is preserved in mean and realisations. 
The random angle of rotation $\rotangle(\event_r)$ is modelled as a von Mises random variable (see \feq{Eq:VMPDF}) with zero mean $\circmeananly=0$ with respect to x-axis and concentration parameter $\concparam=75$.
% Considering the mean direction of the rotation angle $\rotangle$ which is set at $\circmeananly=0$ with respect to x-axis and concentration parameter $\concparam=75$, the angular parameter $\rotangle(\event_r)$ is modelled as a von Mises random variable (see \feq{Eq:VMPDF}). 
In \ffig{Fig:orthoorthoVM}, the \acrshort{pdf} $f(\rotangle(\event_r))$ is shown on a real line over the domain $(-\pi,\pi]$, whereas the realisations of random variable $\rotangle(\event_r)$ and its sample mean vector (solid straight line) are plotted on a unit circle in \ffig{Fig:orthoorthoVMunit}.
In this study, we model directional uncertainty on the $x-y$ plane with $z$ as the axis of rotation.
Thereby, the corresponding random rotation matrix $\rotmat(\event_r)$ in \feq{Eq:stomodrot} takes the form:
\begin{equation}\label{Eq:Rmatrix}
\rotmat(\event_r) =
\begin{bmatrix}
\cos\rotangle(\event_r) & -\sin\rotangle(\event_r)  \\ \sin\rotangle(\event_r) & \cos\rotangle(\event_r)
\end{bmatrix}.
\end{equation}
Here we consider a right-handed Cartesian coordinate system, meaning that positive values of random variable $\rotangle(\event_r)$ indicate counterclockwise rotation and vice versa.  
 \ffig{Fig:orthoorthorot} depicts the corresponding elliptical geometric visualization of the model.
% For easier visualization, we scale the random orientations in the realisations of all the random tensor models in this study by a factor of 1.5.
As can be seen that the orientation of elliptical semi-axes fluctuates in the realisations $\{\conducttensorrot(\event_{r_i})\}^\samplesize_{i=1}\equiv\{\conducttensor_{r_i}\}^\samplesize_{i=1}$, whereas its size and shape remain constant in the mean and realisations.
\begin{figure}[h!]
%	\begin{subfigure}{0.32\textwidth}
%		\centering
%		\input{images/input/2D_LN_ortho_ortho}
%		\caption{}
%	\end{subfigure}\hspace{0.45cm}
	\begin{subfigure}{0.49\textwidth}
		\centering
		\includegraphics[width=0.7\linewidth]{images/input/2D_VM_pdf_rot.eps} %tex files are too big, hence .eps
		\caption{}
		\label{Fig:orthoorthoVM}
	\end{subfigure}
	\begin{subfigure}{0.49\textwidth}
		\centering
		\includegraphics[width=0.75\linewidth]{images/input/2D_VM_unit_rot.eps}
		\caption{}
		\label{Fig:orthoorthoVMunit}
	\end{subfigure}
%	\caption{(a) Lognormal PDF of eigenvalues $\varLambda_1$ and $\varLambda_2$, (b) von Mises PDF of orientation angle $\rotangleVM$ in Cartesian coordinates, (c) realisations of $\rotangleVM(\event)$ on unit circle with resultant mean vector (red line)}
%	\begin{subfigure}{0.49\textwidth}
%		\centering
%		\input{images/input/2D_ortho_ortho_scl}
%		\caption{}
%	\end{subfigure}
	\begin{subfigure}{\textwidth}
		\centering
		\includegraphics[width=0.7\linewidth]{images/input/2D_ortho_ortho_rot_v2.eps}
		\caption{}
		\label{Fig:orthoorthorot}
	\end{subfigure}
%	\begin{subfigure}{\textwidth}
%		\centering
%		\input{images/input/2D_ortho_ortho_rotscl}
%		\caption{}
%	\end{subfigure}		
	\caption{Stochastic tensor $\conducttensorrot(\event_r)$ with fixed symmetry (\acrshort{ortho}-\acrshort{ortho}-\acrshort{dir}): \subref{Fig:orthoorthoVM} von Mises \acrshort{pdf} of random rotation angle $\rotangle(\event_r)$, \subref{Fig:orthoorthoVMunit}  realisations of circular random variable $\rotangle(\event_r)$ on unit circle with resultant mean vector (solid straight line), \subref{Fig:orthoorthorot}  geometric visualization of reference tensor $\meanconducttensorortho$ and realisations of random tensor $\conducttensorrot(\event_r)$; the geometries are enhanced by scaling the eigenvalues by a factor of 0.5, and the orientations with respect to the mean are scaled by a factor of 1.5}
\end{figure}
